Structural and electrochemical properties of MnO2-Carbon based supercapacitor electrodes

We present results of an approach to incorporate redox-active manganese oxide into the 3-dimensional porous structure of carbon xerogels under self-limiting electroless conditions. By varying the structure of the carbon backbone, we found that deposition of manganese oxide preferably takes place on the external surface area of the carbon xerogels. From our detailed analysis we conclude that 3-dimensional carbon xerogels with particle and pore sizes ranging from 10 to 20 nm and low manganese oxide precursor concentration combined with long deposition times are beneficial for fast operating pseudocapacitance electrodes with high capacitance and effective use of the redox active component.

==> tmpbib.tex <==
[2.] [53][57]
[3.] [2483][2498]
[4.] [937][950]
[5.] [220][223]
[6.] [3184][3190]
[7.] [1240][1248]
[8.] [2579][2585]
[9.] [315][320]
[10.] [A1160][A1165]
[11.] [356][361]
[12.] [120][127]
[13.] [167][176]
[14.] [901][907]
[15.] [281][286]
[16.] [A246][A252]
[17.] [1739][1758]
[18.] [126][130]
[19.] [C27][C32]
[20.] [225606][225606]
[21.] [309][315]
[22.] [319][323]
[23.] [1362][1366]
[24.] [7334][ 7339]
[25.] [2478][2486]
[27.] [2486][2493]
[28.] [221][232]
[29.] [6880][6887]
[30.] [554][556]
[31.] [13786][13795]
[32.] [2381][2386]
[33.] [110][115]
[34.] [2759][2764]
[36.] [6845][6849]

